Adaptive Contract Design for Crowdsourcing Markets: Bandit Algorithms for Repeated Principal-Agent Problems

Crowdsourcing markets have emerged as a popular platform for matching available workers with tasks to complete. The payment for a particular task is typically set by the task's requester, and may be adjusted based on the quality of the completed work, for example, through the use of "bonus" payments. In this paper, we study the requester's problem of dynamically adjusting quality-contingent payments for tasks. We consider a multi-round version of the well-known principal-agent model, whereby in each round a worker makes a strategic choice of the effort level which is not directly observable by the requester. In particular, our formulation significantly generalizes the budget-free online task pricing problems studied in prior work. We treat this problem as a multi-armed bandit problem, with each "arm" representing a potential contract. To cope with the large (and in fact, infinite) number of arms, we propose a new algorithm, AgnosticZooming, which discretizes the contract space into a finite number of regions, effectively treating each region as a single arm. This discretization is adaptively refined, so that more promising regions of the contract space are eventually discretized more finely. We analyze this algorithm, showing that it achieves regret sublinear in the time horizon and substantially improves over non-adaptive discretization (which is the only competing approach in the literature). Our results advance the state of art on several different topics: the theory of crowdsourcing markets, principal-agent problems, multi-armed bandits, and dynamic pricing.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= latex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips -t #letter
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(PDF)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(geteps) ; echo $$epses ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

$(PDF)  : %.pdf : %.dvi
	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
#$(PDF) : %.pdf : %.tex
#	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> app-applications.tex <==
%\section{Applications and special cases: the proofs}
%\label{app:applications}
\newcommand{\HighLowFormat}[1]{{\tt #1}\xspace}
\newcommand{\high}{\HighLowFormat{high}}
\newcommand{\High}{\HighLowFormat{High}}
\newcommand{\low}{\HighLowFormat{low}}
\newcommand{\Low}{\HighLowFormat{Low}}

\newcommand{\cH}{c_{\mathtt{h}}}
\newcommand{\vH}{v_{\mathtt{h}}}
\newcommand{\dH}{D_{\mathtt{h}}}

\section{A special case: the ``\hlexample"}
\label{sec:hlexample}

We show an application of the machinery in Section~\ref{sec:regret-bounds} on a specific example; in particular, on this example \zooming significantly outperforms \NonAdaptive.
 
The most basic special case is when there is just one non-null outcome. Essentially, each worker makes a strategic choice whether to accept or reject a given task (where ``reject" corresponds to the null effort level), and this choice is fully observable. This setting has been studied before \cite{Bobby-focs03,DynProcurement-ec12,Krause-www13,BwK-focs13} under the name \emph{dynamic procurement}. Here the contract is completely specified by the price $p$ for the non-null outcome. The supply distribution is summarized by the function
    $F(p) =\Pr[ \text{accept}|p] $,
so that the corresponding expected utility is $U(p) = F(p)(v-p)$. This special case is already quite subtle; by using adaptive discretization, we achieve significant improvement over prior work; see Appendix~\ref{sec:pricing} for further discussion.
 
 
\OMIT{and  its ``dual,'' \emph{dynamic pricing}, in which the principal is selling rather than buying~\cite{Bobby-focs03,BZ09,DynPricing-ec12,BwK-focs13}. }

\newcommand{\prH}{\theta_{\mathtt{h}}}

We consider a somewhat richer setting in which workers' strategic decisions are \emph{not} observable, a salient feature of \problem called \emph{moral hazard} in the contract theory literature.
There are two non-null outcomes (\low and \high), and two non-null effort levels (\low and \high). \Low outcome brings zero value to the requester, while $\high$ outcome brings a positive value $v$ to the requester. \Low effort level inflicts zero cost on a worker and leads to low outcome with probability $1$. We assume that workers break ties between effort levels in a consistent way: \high better than \low better than {\tt null}. (Hence, as \low effort incurs zero cost, the only possible outcomes are \low and \high.)  We will call this the {\bf\em \hlexample}; it is perhaps the simplest example that features moral hazard.

In this example, the worker's type consists of a pair $(\cH,\prH)$, where $\cH\geq 0$ is the cost for \high effort and $\prH\in[0,1]$ is the probability of \high outcome given \high effort. Note that dynamic procurement is equivalent to the special case $\prH=1$.


\begin{claim}
Consider the \hlexample with a fixed supply distribution. Then 
    $\Pr[\text{\high outcome} \,|\, \text{contract $x$}]$
depends only on
    $p = x(\high)-x(\low)$;
denote this probability by $F(p)$. It follows that the expected utility is 
    $U(x) = F(p) (v - p) - x(\low)$.
\label{claim:hlexample}
\end{claim}

For our purposes, the supply distribution is summarized via the function $F(\cdot)$. Denote $\tilde{U}(p) = F(p) (v - p)$. Note that $U(x)$ is maximized by setting $x(\low)=0$, in which case $U(x) = \tilde{U}(p)$. Thus, if an algorithm knows that it is given a \hlexample, it can set $x(\low)=0$, thereby reducing the dimensionality of the search space. Then, assuming function $F(\cdot)$ is non-decreasing, the problem essentially reduces to dynamic procurement with the same $F(\cdot)$.

However, in general an algorithm does not \emph{know} whether it is presented with the \hlexample (because the effort levels are not observable). So in what follows we will consider algorithms that do not restrict themselves to $x(\low)=0$.

We focus on a supply distribution $D$ that is ``nice", in the sense that $F(\cdot)$ satisfies the following two properties:
\begin{OneLiners}
	\item $F(p)$ is Lipschitz-continuous: $|F(p) - F(p')| \leq L |p-p'|$  for some constant $L$.
	\item $\tilde{U}(p)$ is \emph{strongly concave}, in the sense that $\tilde{U}''(\cdot)$ exists and satisfies $\tilde{U}''(\cdot)\leq C<0$.
\end{OneLiners}
Here $L$ and $C$ are absolute constants.
We call such $D$ \emph{strongly Lipschitz-concave}.

The above properties are fairly natural. For example, they are satisfied if $\prH$ is constant and the marginal distribution of $\cH$ is piecewise uniform such that the density is between $\tfrac{1}{\lambda}$ and $\lambda$, for some absolute constant $\lambda\geq 1$.

We show that \zooming has a small width dimension in this setting, and therefore small regret. This holds for any choice $\Xcand\subset X$; in particular, \zooming achieves this without knowing that it is presented with the \hlexample.


\begin{lemma}
Consider the \hlexample with a strongly Lipschitz-concave supply distribution. Then the width dimension is at most $\tfrac12$, for any given $\Xcand\subset X$.
Therefore, \zooming with this $\Xcand$ has regret $R(T|\Xcand) = O(\log T)\, T^{3/5}$.
\label{lm:concave}
\end{lemma}

We contrast this with the performance of \NonAdaptive, parameterized with the natural choice of $\Xcand = \Xcand(\minSize)$, the set of all bounded, monotone contracts with payments that are integer multiples of a given $\minSize>0$. We focus on regret $R(T|X)$, i.e. regret w.r.t. an unrestricted contract in $X$. We show that \zooming achieves regret $R(T|X) = \tildeO{T^{3/5}}$ for a wide range of $\Xcand$, whereas \NonAdaptive cannot do better than
    $R(T|X) = O(T^{2/3})$
for any $\Xcand = \Xcand(\minSize)$, $\minSize>0$.

\begin{lemma}
Consider the setting of Lemma~\ref{lm:concave}. Then: 
\begin{OneLiners}
\item[(a)] \zooming with $\Xcand \supset \Xcand(T^{-2/5})$ has regret $R(T|X) = O(T^{3/5}\, \log T)$.
\item[(b)] \NonAdaptive with $\Xcand = \Xcand(\minSize)$ cannot achieve regret
    $R(T|X)< o(T^{2/3})$
    over all problem instances, for any $\minSize>0$.
\end{OneLiners}
\label{claim:concave}
\end{lemma}

\OMIT{
Moreover, the $T^{2/3}$ lower bound holds even if \NonAdaptive is tuned to the \hlexample so that 
    $\Xcand = \{ x\in \Xcand(\psi):\, x(\low)=0 \}$. 
}    



==> contract_space.tex <==
%
% Contents of this file have been merged into algorithm.tex
%
%




==> pricing-selling.tex <==
\section{Application to dynamic inventory pricing}
\label{app:pricing-selling}

We consider the \emph{dynamic inventory-pricing}, the ``dual'' version of \taskPricing in which the principal is selling rather than buying~\cite{Bobby-focs03,BZ09,DynPricing-ec12,BwK-focs13}.%
\footnote{The ``selling" version is usually called ``dynamic pricing" in the literature; we term it ``dynamic inventory-pricing" to emphasize the distinction between buying and selling.}

The basic version of dynamic inventory-pricing is as follows. In each round $t$, an agent (buyer) arrives. The principal offers one item for sale at price $p_t$. The agent buys if and only if $p_t\leq v_t$, where $v_t\in[0,1]$ is the agent's value for an item. Like in \taskPricing, the value $v_t$ is \emph{private} (not known to the principal). Each value $v_t$ is sampled independently from a fixed distribution, called the \emph{demand distribution}. We consider the prior-independent case in which the demand distribution is not known to the principal. The principal's utility is simply the total payment; the principal has no supply contracts and derives no value from left-over items. The algorithm's goal is to choose the offered prices $p_t$ so as to optimize the expected utility of the principal.
This problem has been addressed in~\citet{Bobby-focs03}, achieving precisely the results as described above for \taskPricing.

Dynamic inventory-pricing can be cast as a special case of the \problem problem. Namely, it is the case of two outcomes (with the non-null outcome corresponding to a sale), where the principal's value is $0$ and (by abuse of notation) the payments are negative. However, negative payments invalidate Lemma~\ref{lm:virtual_width}, and necessitate a different (but very natural) definition of virtual width. Recall that a cell $C$ in this setting is simply an interval $[p^-, p^+]\in [0,1]$, where (if $C$ is composite) $p^-$ and $p^+$ are the two anchors. Let $S(p)$ be the probability of the non-null outcome (i.e, a sale) at price $p$; note that $S(p)$ is  non-increasing in $p$. We define the two-outcome version of virtual width as
\begin{align}\label{eq:virt-width-pricing}
\vw_2(C) = p^+\cdot S(p^-) - p^- \cdot S(p^+).
\end{align}
It is easy to see that
    $\width(C) \leq \vw_2(C)$.
Thus, \zooming and analysis thereof carry over word-by-word.
% We omit the easy modifications from this version.
In particular, Theorem~\ref{thm:procurement} applies word-by-word to dynamic inventory-pricing, with $(k,\lambda)$-uniform costs replaced by with $(k,\lambda)$-uniform values (which are defined in a similar way).

\begin{theorem}\label{thm:pricing}
Consider the dynamic inventory-pricing problem with $(k,\lambda)$-uniform values.
\zooming with $\Xcand=X$ achieves regret
    $R(T) = \tildeO(\min( \lambda^{1/3} T^{2/3},\,
        \lambda^{3/5} k^{2/5} T^{3/5}))$.
\end{theorem}


Further, the lower bounds for \NonAdaptive (Lemma~\ref{lm:procurement-NonAdaptive}) carry over, too.
The constructions used in the proof of Lemma~\ref{lm:pricing-NonAdaptive} are similar to those in the proof of Lemma~\ref{lm:procurement-NonAdaptive}, but slightly different technically. We omit the details.

\begin{lemma}\label{lm:pricing-NonAdaptive}
Consider dynamic inventory-pricing problem $(k,4)$-uniform costs.
\begin{OneLiners}
\item[(a)]
    $R_\minSize(T) = \Omega(\minSize T + \minSize^{-2}) \geq \Omega(T^{2/3})$.

\item[(b)] $\NonAdaptive(\minSize)$ achieves regret $R(T)=\Omega(T^{2/3})$ for $\minSize = \tildeO(T^{-1/3})$, even if $k=2$.

\end{OneLiners}
\end{lemma}




==> prior_space.tex <==
In this section, we explore the contract menu design problem and relax the full information
setting. In particular, we assume we know agent cost function $c_i(\cdot)$
and agent output conditional probability $f_i(\pi|e_i)$. But the agent prior distribution 
$\{\lambda_i\}$ is unknown. We also assume there are the number of output qualities and 
the number of effort levels are both finite.

Note that if $\{\lambda_i\}$ is also known, we can obtain the optimal contract menu by solving
the linear program of the contract menu design problem. Therefore, in this setting, instead of 
directly finding optimal contract menus, we can also choose to estimate true agent prior first and
then solve the optimal contract menu. This might simplify the problem since the dimension
of agent priors is smaller than the dimension of contract menus.

\subsection{Bandit Formulation: Search over Prior Space}

We can formulate the setting with unknown priors as a bandit 
problem. Each arm corresponds to an instance of prior distribution. 
After selecting an arm/prior, we can calculate the optimal contract given this prior.
The reward of the arm is the principal's payoff for posting the corresponding contract.


\subsubsection{(Weak) Lipschitz condition}
\ignore{
We show that if we post a contract which is determined by solving the linear
program of the contract menu design problem using estimated agent prior, 
as long as the estimated prior is not too far way from 
the real prior, our contract also generates rewards close to the optimal contract.}

Below we show that this problem is actually a Lipschitz MAB problem. We prove the (weak)
Lipschitz condition, i.e., if the selected prior is not too far way from the real prior, the reward
we get is also not too far away from the optimal reward. 


\begin{lemma}
Let $\vec{\lambda}^*$ be the true prior and $\vec{\lambda}'$ be an estimated prior. 
Also let $u(\vec{\lambda}^*)$ and $u(\vec{\lambda}')$ be the expected payoff the 
principal receives by choosing arms $\vec{\lambda}^*$ and $\vec{\lambda}'$, we have
\[
\abs{u(\vec{\lambda}^*) - u(\vec{\lambda'})} \leq C \|\vec{\lambda}^*-\vec{\lambda}'\|_1, 
\]
where $C=\max_{\{i,\vec{\lambda}\}} h_i(\vec{\lambda})-\min_{\{i,\vec{\lambda}\}} h_i(\vec{\lambda})$.
\end{lemma}
\begin{proof}
Let $\vec{h}^* = \{h^*_i\}$ be the vector of expected principal payoff, 
in which each dimension $h^*_i$
represents the payoff the principal gets from an agent of type $i$ when posting the contract
by solving the contract menu design problem with $\vec{\lambda}^*$.
In this case, the expected payoff received by the principal is the inner product of both vectors:
$u(\vec{\lambda}^*) = \vec{\lambda}^*\cdot\vec{h}^*$.

Similarly, let $\{\lambda'_i\}$ be an estimated prior and $\vec{h}'$ be the corresponding payoff 
vector. The expected payoff received by the principal
$u(\vec{\lambda}') = \vec{\lambda}^*\cdot\vec{h'}$ 
(the expected payoff is still realized by true prior.) 

Note that in the contract menu design problem, agent prior $\{\lambda_i\}$ only appears in the 
objective function. Therefore, the set of feasible solutions is the same no matter 
which agent prior we choose. Also, since $\vec{h}'$ is generated from the optimal solution
with $\vec{\lambda}'$, we have 
\[
	\vec{\lambda}' \cdot \vec{h}' \geq \vec{\lambda}' \cdot{h}^*.
\]

Given the above inequality, we can complete the proof as follows.
\begin{align*}
	u(\vec{\lambda}^*) - u(\vec{\lambda}')
	&= \vec{\lambda}^*\cdot\vec{h}^*-\vec{\lambda}^*\cdot\vec{h}' 	 \\
	&= \vec{\lambda}^*\cdot\vec{h}^* - \vec{\lambda}^*\cdot\vec{h}' + \vec{\lambda}'\cdot\vec{h}' - \vec{\lambda}'\cdot\vec{h}' \\ 
	&\leq \vec{\lambda}^*\cdot\vec{h}^* - \vec{\lambda}^*\cdot\vec{h}' + \vec{\lambda}'\cdot\vec{h}' - \vec{\lambda}'\cdot\vec{h}^* \\ 
	&= (\vec{\lambda}^*-\vec{\lambda}')\cdot\vec{h}^* - (\vec{\lambda}^*-\vec{\lambda}')\cdot\vec{h}' \\
	&= (\vec{\lambda}^*-\vec{\lambda}')\cdot(\vec{h}^*-\vec{h}') \\
	&\leq \left(\max_{i,\vec{\lambda}} h_i(\vec{\lambda}) -  \min_{i,\vec{\lambda}} h_i(\vec{\lambda})\right) \| \vec{\lambda}^*-\vec{\lambda}|\|_1
\end{align*}

\end{proof}
If we assume we have prior information of $\max_{\{i,\vec{\lambda}\}} h_i(\vec{\lambda})$ and 
$\min_{\{i,\vec{\lambda}\}} h_i(\vec{\lambda})$. We can treat them as constants and obtain
the weak Lipschitz condition.

\subsubsection{Brief discussion on full feedback}

Note that if we always design feasible contracts (i.e., feasible solution of the linear program),
agents will always choose their own contracts, and the principal will know which type is
arriving. It's equivalent to have full feedback (we know what would happen if we choose a 
different feasible contract.)

Below we illustrate a simple algorithm which empirically estimates agent prior,
solves the linear program by using the estimated prior, and posts the corresponding contract
in each round. Below we very roughly estimate the regret of this algorithm.

Note that after round t, the prior estimation error for each agent type is 
bounded by $O(1/\sqrt{t})$ with high probability (if we use empirical mean and Hoeffding bound.) 

Given the weak Lipschitz condition, if we choose the contract by solving the linear program using 
estimated prior, our payoff is not too far away from the optimal payoff (i.e., bounded 
by $O(n/\sqrt{t})$, the one-norm distance between estimated prior and optimal prior.)

So the total regret after round T would be $\sum_{t=1}^T O(n/\sqrt{t}) = O(n \sqrt{T})$.

\cj{discussion of uncertain agent type parameters}


==> zooming.tex <==

A.S.: OBSOLETE FILE, WE ARE NOT USING IT ANY MORE!!


